Terahertz transitions in finite carbon chains

We predict an optical effect associated with systems which exhibit topologically protected states separated by a finite distance. We develop a tight-binding model to calculate the optical selection rules in linear chains of atoms of different lengths, and show the crucial importance of edge states. For long enough molecules the interband transitions involving these edge states are in the highly sought-after THz frequency range. Although we have specifically considered finite carbon chains terminated by gold nanoparticles, the main results of our work can be generalized to various systems which exhibit topologically protected states separated by a finite distance.

==> spare.tex <==


%It should be noted that within the tight-binding model the presence of aligned structures can lead to the change in the band gap due to inter-chain interaction. 

%The broadening of the single carbon bond peak is explained by the fact that this bond is weaker than the other one.


%Gold anchors offer several important advantages for practical applications of carbon chains. 

%Gold stabilise the polyyne allotrope of carbyne. 

%The gold anchors strongly reduce the negative role of Peierls deformations allowing for the deposition of record-long straight linear carbon chains without any supplementary stabilisation.


For the polarization vector along the chain, the transition dipole moment for our system is given by the expression:
\begin{equation}
\left\langle \psi_{f}\left|\hat{\boldsymbol{e}}\cdot{\boldsymbol{r}}\right|\psi_{i}\right\rangle =\sum_{j=1,\,3,\,5,\,\ldots}^{N-1}u_{j}^{p}u_{j}^{p'}\frac{\left(j-1\right)c}{2}
+
\sum_{j=2,\,4,\,6,\,\ldots}^{N}u_{j}^{p}u_{j}^{p'}\left(\frac{jc}{2}-c_{s}\right),
\label{eq:transition}
\end{equation}
where $u_{j}^{p}$ and $u_{j}^{p'}$ are the $j^{th}$ components of the eigenvectors of the initial and final states given in Eq~(\ref{evector_1}) and Eq~(\ref{evector_2}). In our notation the HOMO and LUMO levels correspond to $p=\frac{1}{2}N$, and $p=\frac{1}{2}N+1$, respectively. 





\subsubsection{Check}
To demonstrate the presence of longer chains, the pump wavelength and spectral range of the photodetector must be carefully tuned. Using the tight-binding parameters comparable to those reported in the literature~\cite{al2014electronic}, for short chains, the separation between energy levels is too small (AK: for a chain of which length?) for an electron to be able to absorb a photon of wavelength 370 nm, relax, and then emit in the range of 444 nm. However, this can occur in much longer chains (AK: much longer than what?). Therefore, our selected wavelengths are ideal to demonstrate the presence of the highly desirable, long chains (AK: any proof of it?). Let us first consider the case where radiation from the pump promotes electrons from the level $p$ to the level $p'=p + 5$. In this instance, the transitions where $p=\frac{1}{2}N-4$ and  $p=\frac{1}{2}N$, shown in Fig. \ref{figure4}d by the blue arrows, fall within the range of 370 nm for chains of length 30, 32, 34 and 36. Depending on the doping, the transition from $p=\frac{1}{2}N -6$ to  $p'=-1$ can also occur. Although this transition falls within the desired range, the strength of the matrix element of optical transition is an order of magnitude less than the strength of the other transitions (AK: which ones?) and hence, this transition shall not be considered here. It should be noted that other shorter length chains can absorb in our wavelength range, if we cosider the  transitions $p$ to $p'=p + 3$. However, although they absorb in the right range, any subsequent relaxation followed by the emission will fall beyond the spectral range of the detector (AK: what is this range?). After the electron is promoted to one of the higher energy levels, there is a variety of possible luminescence channels. All the transitions corresponding to $p'=p - 1$ are outside the detector range, whereas only the transitions from  $p'=p - 3$ are within the range.  It should be noted that for long chains (AK: how long?), the transition between the edge-states is approximately one order of magnitude less efficient than other $p'=p - 1$ transitions. 

Let us first consider the relaxation paths associated with an electron promoted from $p=\frac{1}{2}N$ to $p'=\frac{1}{2}N +5$. The matrix element of the transition for $p=\frac{1}{2}N+3$ to $p'=\frac{1}{2}N$ (towards the red side of the spectrum) and $p=\frac{1}{2}N+4$ to $p'=\frac{1}{2}N+1$ (towards the blue side of the spectrum) are much stronger than for $p=\frac{1}{2}N+5$ to $p'=\frac{1}{2}N+2$. The absence of prominent peaks and the monotonic decrease in the intensity of photoluminescence towards the red can be explained by electron-doping. The laser synthesis of colloidal particles results in the charging of the gold nanoparticles~\cite{kucherik2017cavitation}. The presence of an additional electron in a chain would suppress the $p=\frac{1}{2}N+3$ to $p'=\frac{1}{2}N$ transition, since electrons from the $\frac{1}{2}N+1$ level would relax to fill the hole generated by the initial excitation. Consequently, the $p=\frac{1}{2}N+4$ to $p'=\frac{1}{2}N+1$ is expected to dominate the photoluminescence spectrum. An electron doping would also suppress the relaxation paths associated with an electron promoted from $p=\frac{1}{2}N - 4$ to $p'=\frac{1}{2}N + 1$. The matrix element of transition for $p=\frac{1}{2}N+1$ to $p'=\frac{1}{2}N-2$ (towards the red side of the spectrum) and $p=\frac{1}{2}N$ to $p'=\frac{1}{2}N-3$ (towards the blue side of the spectrum) are considerably stronger than for $p=\frac{1}{2}N-1$ to $p'=\frac{1}{2}N-4$. For an electron to relax from $p=\frac{1}{2}N$ to $p'=\frac{1}{2}N-3$, a hole must migrate from $p=\frac{1}{2}N - 4$ to $p=\frac{1}{2}N - 3$. Whereas for an electron to relax from $p=\frac{1}{2}N+1$ to $p'=\frac{1}{2}N-2$, a hole must undergo two transitions upwards. Therefore, the blue transitions dominate the spectrum. It should be noted that although the transition between $p=\frac{1}{2}N +2 $ to $p=\frac{1}{2}N - 1$ is in the correct range associated with the prominent peaks, it would require  the absorption of two photons, and several hole transitions, and therefore only weakly contributes to the overall observed photoluminescence spectrum. 


The matrix element of the optical transition monotonically increases with wavelength. However, the probability of synthesis decreases with the increase of the number of atoms in a chain that results in the overall reduction of the absorbance with the increase of the wavelength.


%By decomposing the wavevector into two components one along the tube axis and one perpendicular to it, and by applying the periodic boundary condition to the momentum directed along the circumferential direction. 
%By using a simple zone folding model, the approximate band structure of a carbon nanotube can be obtained from the band structure of graphene along allowed lines in k-space defined by the chiral vector\cite{dresselhaus1998physical}.

Symmetric stretch, Antisymmetric stretch, bends etc. which ...




Natural broadening - Result of finite radiative lifetime

Collisional/pressure broadening - Finite lifetime in quantum state owing to collisions

Doppler broadening - Thermal motion






Doppler and Pressure Broadening. 

Doppler broadening

Pressure Broadening, A second type of broadening occurs due to the interaction of collisions with the absorbing medium. The broadening, known as pressure or collisional broadening increases linearly with the collision rate (and thus to first order
pressure). The line shape is quite different from the Doppler shape (Lorentzian):
where  is the pressure broadened width, and  is the distance from line
center. The Lorentzian line shape is much broader producing significant absorption
far from line center.

